Families of vector fields with many numerical invariants

We study bifurcations in finite-parameter families of vector fields on $S^2$. Recent papers by Yu. Ilyashenko, N. Goncharuk, Yu. Kudryashov, I. Schurov, and N. Solodovnikov provide examples of (locally generic) structurally unstable families of 3-parameter vector fields: generic close 3-parameter families experience different bifurcations. In this paper, we use these results to construct new examples of few-parameter generic families of planar vector fields such that their classification has many invariants. In particular, we construct (a) 3-parameter families with infinitely many numerical invariants; (b) 4-parameter families with arbitrarily many "robust" numerical invariants; (c) 5-parameter families with functional invariants.

==> asy/many-invariants-1.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-1_0}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-136.391467,73.491748)(-0.292893,-1.000000){ }%


==> asy/many-invariants-2.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-2_0}%
}%


==> asy/many-invariants-3.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-3_0}%
}%


==> asy/many-invariants-4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-4_0}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-84.114356,68.405423)(0.000000,-0.500000){\(c\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-110.594448,70.534698)(-1.000000,0.179999){\(L_1\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-63.656763,70.534698)(0.000000,0.179999){\(R_1\)}%


==> asy/many-invariants-5.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-5_0}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-87.561412,3.387656)(-0.500000,0.000000){\(b\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-149.450837,83.605399)(0.000000,-0.820001){\(S_1\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-25.671986,83.605399)(-1.000000,-0.820001){\(S_2\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-127.229296,43.055540)(0.000000,-0.320001){\(\Gamma_1\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-47.893528,43.055540)(-1.000000,-0.320001){\(\Gamma_2\)}%


==> asy/many-invariants-6.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-6_0}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-87.561412,3.387656)(-0.500000,0.000000){\(b\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-149.450837,87.863949)(0.000000,0.179999){\(S_1\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-25.671986,87.863949)(-1.000000,0.179999){\(S_2\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-119.570762,102.806328)(-0.500000,-0.500000){\(s\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-83.044537,119.877981)(0.000000,-0.500000){\(R\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-89.690687,79.337485)(-1.000000,-0.820001){\(L_1\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-89.690687,57.997918)(-1.000000,-0.820001){\(L_2\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-89.690687,32.390438)(-1.000000,-0.820001){\(L_3\)}%


==> asy/many-invariants-7.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-7_0}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-121.563223,107.074241)(-0.500000,-0.500000){\(s\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-123.692499,75.069572)(-1.000000,-0.736690){\(l_2^s=l_2^u\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-25.535172,95.147794)(-0.500000,0.258371){\(u_2\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-25.535172,84.857381)(-0.500000,-0.741629){\(u_3\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-85.036998,124.145894)(0.000000,-0.500000){\(R\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-91.683148,62.265832)(-1.000000,-0.820001){\(L_2\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-91.683148,36.658351)(-1.000000,-0.820001){\(L_3\)}%

